GD-1 Stellar Stream and Cocoon in the DESI Early Data Release

We present 115 new spectroscopically identified members of the GD-1 tidal stream observed with the 5000-fiber Dark Energy Spectroscopic Instrument (DESI). We confirm the existence of a ``cocoon'' which is a broad (FWHM~2.932 deg ~ 460 pc) and kinematically hot (velocity dispersion, sigma ~ 5-8 km/s) component that surrounds a narrower (FWHM~ 0.353 deg ~ 55) and colder (sigma = 3.09+/-0.76 km/s) thin stream component (based on a median per star velocity precision of 2.7 km/s). The cocoon extends over at least a 30 degree segment of the stream observed by DESI. The thin and cocoon components have similar mean values of [Fe/H]: -2.54+/- 0.04 dex and -2.47+/- 0.06 dex suggestive of a common origin. The data are consistent with the following scenarios for the origin of the cocoon. The progenitor of the GD-1 stream was an accreted globular cluster (GC) and: (a) the cocoon was produced by pre-accretion tidal stripping of the GC while it was still inside its parent dwarf galaxy; (b) the cocoon is debris from the parent dwarf galaxy; (c) an initially thin GC tidal stream was heated by impacts from dark subhalos in the Milky Way; (d) an initially thin GC stream was heated by a massive Sagittarius dwarf galaxy; or a combination of some these. Future DESI spectroscopy and detailed modeling may enable us to distinguish between these possible origins.

==> table_phi1_splines.tex <==




